MAMMOTH: Massively Multilingual Modular Open Translation @ Helsinki

NLP in the age of monolithic large language models is approaching its limits in terms of size and information that can be handled. The trend goes to modularization, a necessary step into the direction of designing smaller sub-networks and components with specialized functionality. In this paper, we present the MAMMOTH toolkit: a framework designed for training massively multilingual modular machine translation systems at scale, initially derived from OpenNMT-py and then adapted to ensure efficient training across computation clusters. We showcase its efficiency across clusters of A100 and V100 NVIDIA GPUs, and discuss our design philosophy and plans for future information. The toolkit is publicly available online.

==> mammoth-emoji.tex <==
🦣


==> video_script.tex <==
--------> (Show paper on background)

Hello everyone,

My name is Joseph Attieh and today I'll present to you our toolkit for Massively Multilingual Modular Open Translation, Mammoth.

Mammoth is a framework designed for training massively multilingual modular machine translation systems at scale, initially derived from
OpenNMT-py and then adapted to ensure efficient training across computation clusters.

Our code is publicly available online in our GitHub. 


------> GO TO GITHUB

We also provide extended documentation in our docs.

------> GO TO DOCS
Show images blabla modularity 
Quickstart

----> GO TO SHOW CODE
0. Show config
1. Train
2. Infer
